Text-Conditioned Sampling Framework for Text-to-Image Generation with Masked Generative Models

Token-based masked generative models are gaining popularity for their fast inference time with parallel decoding. While recent token-based approaches achieve competitive performance to diffusion-based models, their generation performance is still suboptimal as they sample multiple tokens simultaneously without considering the dependence among them. We empirically investigate this problem and propose a learnable sampling model, Text-Conditioned Token Selection (TCTS), to select optimal tokens via localized supervision with text information. TCTS improves not only the image quality but also the semantic alignment of the generated images with the given texts. To further improve the image quality, we introduce a cohesive sampling strategy, Frequency Adaptive Sampling (FAS), to each group of tokens divided according to the self-attention maps. We validate the efficacy of TCTS combined with FAS with various generative tasks, demonstrating that it significantly outperforms the baselines in image-text alignment and image quality. Our text-conditioned sampling framework further reduces the original inference time by more than 50% without modifying the original generative model.

==> contents/Trade-off.tex <==
\begin{figure}[t]
    \includegraphics[width=1\linewidth]{figures/figure2_temp.pdf}
    \centering
     % \caption{\small CLIP score, FID trade-off graph with 30K text-image pairs from MS-COCO dataset.  On average, samples by uniform sampling have better quality but tend to have poor text-alignment. On the other hand, regrettable sampling, such as random revoke, is advantageous for text-alignment by obtaining more recovery opportunities, but the image quality is degraded due to unstable sampling.}
     \caption{\small MID, FID trade-off graph with 30K text-image pairs from MS-COCO dataset.  On average, samples by uniform sampling have better quality but tend to have poor text-alignment. On the other hand, regrettable sampling, such as random revoke, is advantageous for text-alignment by obtaining more recovery opportunities, but the image quality is degraded due to unstable sampling.}
    %\label{tradeoff}
\end{figure}
% 우리 모델도 Fixed schedule로 사용하면 FID는 좋아지지만, MID 낮아짐, 다른 hyperparameter들로 trade-off도 있지만, Fixed vs Revocable이 MID의 trade-off에 큰 영향을 끼치는 것을 확인할 수 있음 > 새 metric (gg3t5로 교체중)

==> contents/archit.tex <==
\begin{figure}[h]
\centering
\vspace{0.2in}
    \includegraphics[width=0.8\linewidth]{figures/trans.pdf}
     \caption{\small \textbf{TCTS inference score at the same time step.} \textbf{Top}: Score from Unet-based model, \textbf{Bottom}: Score from Transformer-based model.}
    %\label{fig:architect}
\end{figure}

==> contents/step.tex <==
\begin{figure*}[t]
\centering
    \includegraphics[height=5cm, width=15cm]{figures/step.png}
     \caption{\small \textbf{step samples} TBD.}
    %\label{fig:step}
\end{figure*}

==> tables/RR.tex <==
\begin{figure}[t]
\vspace{-0.15in}
\begin{minipage}{\linewidth}
\centering
\begin{algorithm}[H]
    \small
    \caption{Random revoke sampling strategy}
	\label{algo:algorithm_rr}
	\begin{algorithmic}[1]
            \STATE $k_t$ tokens are sampled at step $t$   $(t = T, T-1,..., 1)$
            \STATE
            \STATE $x_T \leftarrow [$[MASK]$]_N$
            \STATE $L = \{0, 1, ..., N-1\}$
            \STATE $\mathcal{U}(I=i|i \in L) = 1/N \leftarrow $ uniform distribution
	    \FOR {$t = T, T-1, ..., 1$}
                \STATE $\hat{x}_0 = G_\theta(x_t,c)$
                % \STATE $A_t = \{i|x_t^i=$[MASK]$\}$
                \STATE $m = k_T + k_{T-1} + ... + k_t$
                \STATE $i_1, i_2, ..., i_m \sim \mathcal{U}(I) \leftarrow $ sample without replacement
                \STATE $x_t \leftarrow[$[MASK]$]_N$
                \FOR {$i = i_1, i_2, ..., i_m$}
                    \STATE $x^i_t \leftarrow \hat{x}^i_0$
                \ENDFOR
            \ENDFOR
        \end{algorithmic}
    \end{algorithm}
\end{minipage}
\vspace{-0.1in}
\end{figure}


==> tables/TC_train.tex <==
\begin{figure}[ht!]
\vspace{-0.1in}
\begin{minipage}{\linewidth}
\centering
\begin{algorithm}[H]
    \small
    \caption{TCTS Training}
	\label{algo:algorithm_tcts}
	\begin{algorithmic}[1]
            \INPUT Pre-trained generator $G_\theta$, text condition $c$
            \OUTPUT Token-Critic parameters $\phi$
            \STATE \textbf{repeat}
            \STATE $x_{0},c \leftarrow $ i.i.d sampled VQ image
            \STATE $t \sim \mathcal{U}_{(0,1)}$
            \STATE $x_t \leftarrow $ sample from $ q(x_t|x_0)$ 
            \STATE $\hat{x}_0 \leftarrow G_\theta(x_t, c)$   \ \ \  /* sampling cf-guidance scale $w \sim \mathcal{U}_{(1,5)}$*/
            \STATE $m_t \leftarrow \{i|x_t^i = $ [MASK]$\}$ 
            \IF {$I \sim \mathcal{U}_{(0,1)} < 0.1 $}
                \STATE $\phi \leftarrow \phi - \eta \bigtriangledown_\phi BCE(m_t,p_\phi(m_t|\hat{x}_0,\emptyset))$ 
            \ELSE 
                \STATE $\phi \leftarrow \phi - \eta \bigtriangledown_\phi BCE(m_t,p_\phi(m_t|\hat{x}_0,c))$ 
            \ENDIF
            \STATE \textbf{until} converged
        \end{algorithmic}
    \end{algorithm}
\end{minipage}
\vspace{-0.2in}
\end{figure}


==> tables/TI_eval.tex <==
\begin{table}[h]
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lccc}
    \toprule
    Model & MID $\uparrow$ & SOA-I $\uparrow$ & FID-30K $\downarrow$ \\
    \midrule
    GLIDE \cite{nichol2021glide} & 1.03 & - & 32.08 \\
    AttnGAN \cite{xu2018attngan} & -65.20 & 39.01 & 29.15 \\
    DM-GAN \cite{lee2022draft} & -44.66 & 48.03 & 22.90 \\
    DF-GAN \cite{tao2020df} & -58.75 & - & 31.75 \\
    VQ-Diffusion \cite{yu2021vector} & -19.63 & - & 13.13 \\
    LAFITE \cite{zhou2022towards} & 6.26 & 74.78 & 8.03 \\
    \midrule
    \textbf{TCTS w/o Attn} & 14.61 & 79.59 & 14.75 \\
    \textbf{TCTS w/ Attn} & 13.99 & 77.28 & 18.93 \\
    \bottomrule
    \end{tabular}}
\vspace{-0.05in}
    \caption{\small Evaluation of TCTS compared to other text-to-image generative models on MS-COCO dataset.}
    %\label{Metric}
\end{table}


==> tables/refine_table.tex <==
\begin{table}[h]
    \centering
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{lcccc}
    \toprule
    Model & MID $\uparrow$ & CLIP-S $\uparrow$ & SOA $\uparrow$ & FID $\downarrow$ \\
    \midrule
    ImageBART \cite{esser2021imagebart} & $11.6$ & $225$ & $3.87$ & $1$ \\
    VQ-Diffusion(U) \cite{gu2022vector} & $2.43$ & $16$ & $0.82$ & $1$ \\
    VQ-Diffusion(P) \cite{gu2022vector} & $2.13$ & $61$ & $1.52$ & $1$ \\
    LDM \cite{rombach2022high} & $11.6$ & $225$ & $3.87$ & $1$ \\
    RQ-Transformer \cite{lee2022autoregressive} & $11.6$ & $225$ & $3.87$ & $1$ \\
    Draft-and-Revise \cite{lee2022draft} & $11.6$ & $225$ & $3.87$ & $1$ \\
    \midrule
    Uniform (16 step) & $2.13$ & $61$ & $1.52$ & $1$ \\
    Uniform (25 step) & $2.13$ & $61$ & $1.52$ & $1$ \\
    Purity (16 step) & $2.13$ & $61$ & $1.52$ & $1$ \\
    Purity (25 step) & $2.13$ & $61$ & $1.52$ & $1$ \\
    \midrule
    \textbf{TCTS} & $\mathbf{1.84}$ & $\mathbf{100}$ & $\mathbf{2.87}$ & $\mathbf{1}$ \\
    \textbf{TCTS + Attn} & $\mathbf{1.84}$ & $\mathbf{100}$ & $\mathbf{2.87}$ & $\mathbf{1}$ \\
    \bottomrule
    \end{tabular}
    }
    \caption{Qualitative evaluation of text-to-image generation on MS-COCO dataset. SOA is calculated in a piece-wise form that has been used in \citealp{kim2022mutual}.}
\end{table}


==> tables/uniform.tex <==
\begin{minipage}[t!]{\linewidth}
% \vspace{-0.1in}
\begin{algorithm}[H]
    \small
    \caption{Uniform sampling strategy}
	%\label{algo:algorithm1}
	\begin{algorithmic}[1]
            \STATE $k_t$ tokens are sampled at step $t$   $(t = T, T-1,..., 1)$
            \STATE
            \STATE $x_T \leftarrow [$[MASK]$]_N$
	    \FOR {$t = T, T-1, ..., 1$}
                \STATE $\hat{x}_0 = G_\theta(x_t,c)$
                \STATE $A_t = \{i|x_t^i=$[MASK]$\}$
                \STATE $\mathcal{U}_t(I=i|i \in A_t) = 1/n(A_t) \leftarrow $ uniform distribution
                \STATE $i_1, i_2, ..., i_{k_t} \sim \mathcal{U}_t(I) \leftarrow $ sample without replacement
                \FOR {$i = i_1, i_2, ..., i_{k_t}$}
                    \STATE $x^i_t \leftarrow \hat{x}^i_0$
                \ENDFOR
            \ENDFOR
    \end{algorithmic}
    \end{algorithm}
\end{minipage}\\

